The State and Future of Genetic Improvement

We report the discussion session at the sixth international Genetic Improvement workshop, GI-2019 @ ICSE, which was held as part of the 41st ACM/IEEE International Conference on Software Engineering on Tuesday 28th May 2019. Topics included GI representations, the maintainability of evolved code, automated software testing, future areas of GI research, such as co-evolution, and existing GI tools and benchmarks.

==> author.tex <==

 %Modifications:
 %WBL 21 Jun 2019 Add whitequeen

\href{http://www.cs.ucl.ac.uk/staff/W.Langdon/}
{William B. Langdon} & 
\href{http://web.eecs.umich.edu/~weimerw/}
{Westley Weimer} & %Westley Weimer weimerw@umich.edu Wed, Jun 12, 2019 at 4:17 PM
\href{https://www.cs.cmu.edu/directory/ctimperl}
{Christopher Timperley} & %christimperley@googlemail.com Wed, Jun 12, 2019 at 3:04 PM
\href{https://aist.fh-hagenberg.at/index.php/en/team-2/oliver-krauss-2}
{Oliver  Krauss} %Oliver.Krauss@fh-hagenberg.at> Thu, Jun 13, 2019 at 3:42 PM
\\
\href{https://www.linkedin.com/in/zhen-yu-ding-23a389155}
{Zhen Yu Ding} & %Zhen Yu Ding <zhenyudg@live.com> Tue, Jun 11, 2019 at 2:12 AM
\href{https://www.cs.cmu.edu/~15210/staff.html#ylyu1}
{Yiwei   Lyu} & %Yiwei Lyu <ylyu1@andrew.cmu.edu> Thu, Jun 13, 2019 at 8:12 PM
Nicolas Chausseau & %nicolas.chausseau@gmail.com Fri, Jun 14, 2019 at 6:26 AM concordia.ca?
\href{http://news.grammatech.com/grammatech-releases-automated-software-engineering-library-into-open-source}
{Eric    Schulte} %eschulte@grammatech.com Mon, Jun 17, 2019 at 6:58 PM
\\
\href{http://www.shinhwei.com/}
{Shin Hwei Tan} & %tansh3@sustc.edu.cn Wed, Jun 12, 2019 at 6:45 PM
\href{http://kjleach.eecs.umich.edu/}
{Kevin Leach} & %Kevin Leach <kjleach@umich.edu> Thu, Jun 13, 2019 at 3:01 PM
\href{http://www-personal.umich.edu/~yhhy/}
{Yu      Huang} & %yhhy@umich.edu Sat, Jun 15, 2019 at 6:52 PM
\href{http://coinse.kaist.ac.kr/members/gabin/}
{Gabin   An} %Gabin An <agb94@kaist.ac.kr> Tue, Jun 18, 2019 at 6:28 AM
\\
\\[2ex]
\multicolumn{4}{c}{\includegraphics[scale=0.5]{pic/whitequeen}}\\
\\[2ex]
\multicolumn{4}{c}{When I was your age I could think of six impossible things before breakfast}

